D3-GNN: Dynamic Distributed Dataflow for Streaming Graph Neural Networks

Graph Neural Network (GNN) models on streaming graphs entail algorithmic challenges to continuously capture its dynamic state, as well as systems challenges to optimize latency, memory, and throughput during both inference and training. We present D3-GNN, the first distributed, hybrid-parallel, streaming GNN system designed to handle real-time graph updates under online query setting. Our system addresses data management, algorithmic, and systems challenges, enabling continuous capturing of the dynamic state of the graph and updating node representations with fault-tolerance and optimal latency, load-balance, and throughput. D3-GNN utilizes streaming GNN aggregators and an unrolled, distributed computation graph architecture to handle cascading graph updates. To counteract data skew and neighborhood explosion issues, we introduce inter-layer and intra-layer windowed forward pass solutions. Experiments on large-scale graph streams demonstrate that D3-GNN achieves high efficiency and scalability. Compared to DGL, D3-GNN achieves a significant throughput improvement of about 76x for streaming workloads. The windowed enhancement further reduces running times by around 10x and message volumes by up to 15x at higher parallelism.

==> reviews/meta-reviews.tex <==
{\noindent\Huge\textbf{Response to Reviewer Comments}}

% 1. Overall Recommendation

%     Revision

% 2. Summary Comments

%     The reviewers agreed on a revision with the main issues to address being writing, scale, and the experimental evaluation. The paper also needs an evaluation on GPUs.

% 3. Revision Items (for "Revision" and "Accept with Shepherding" papers)

%     1. Please perform experiments with GPUs as well.
%     2. From Reviewer 1: Please address comments W1-W3 in Question 7, the issues pointed out in the detailed evaluation, and Question 14.
%     3. From Reviewer 2: Please address D1 through D4
%     4. From Reviewer 3: Please address the issues D1 and D2, and it would be great if you could also address D3 but that is not a must. 
\begin{snugshade*}
\noindent 
Dear Reviewers,

\noindent 
Thank you for your thorough review and valuable suggestions. We appreciate the time and effort you have put into evaluating our work. We have taken your feedback seriously and have conducted additional experiments as requested.

\noindent 
In response to Reviewer \#4's comment, we have incorporated the WikiKG90Mv2 dataset into our study. This dataset, being significantly large and complex, provided an excellent opportunity to test the scalability and performance of our proposed methods.

\noindent 
We have conducted extensive experiments on this dataset using three different windowing algorithms: Sliding, Session, and Adaptive. These experiments were designed to evaluate the robustness and efficiency of our approach under high-load conditions.

\noindent 
The results from these additional experiments have been integrated into our revised manuscript (\autoref{fig:sx_superuser}), and we believe they substantially enhance the comprehensiveness and rigor of our study.

\noindent 
Thank you again for your insightful comments and recommendations. We hope the revisions meet your expectations and look forward to your feedback.

\noindent 
Best regards,

\noindent 
D3-GNN Team

\end{snugshade*}

